Approximating Matrix p-norms

We consider the problem of computing the q->p norm of a matrix A, which is defined for p,q \ge 1, as |A|_{q->p} = max_{x !=0 } |Ax|_p / |x|_q. This is in general a non-convex optimization problem, and is a natural generalization of the well-studied question of computing singular values (this corresponds to p=q=2). Different settings of parameters give rise to a variety of known interesting problems (such as the Grothendieck problem when p=1 and q=\infty). However, very little is understood about the approximability of the problem for different values of p,q. Our first result is an efficient algorithm for computing the q->p norm of matrices with non-negative entries, when q \ge p \ge 1. The algorithm we analyze is based on a natural fixed point iteration, which can be seen as an analog of power iteration for computing eigenvalues. We then present an application of our techniques to the problem of constructing a scheme for oblivious routing in the l_p norm. This makes constructive a recent existential result of Englert and R\"acke [ER] on O(log n)-competitive oblivious routing schemes (which they make constructive only for p=2). On the other hand, when we do not have any restrictions on the entries (such as non-negativity), we prove that the problem is NP-hard to approximate to any constant factor, for 2 < p \le q, and p \le q < 2 (these are precisely the ranges of p,q with p\le q, where constant factor approximations are not known). In this range, our techniques also show that if NP does not have quasi-polynomial time algorithms, the q->p cannot be approximated to a factor 2^{(log n)^{1-eps}}, for any \eps>0.

==> intro.tex <==
\section{Introduction}
Linear operators over finite dimensional vector spaces have been
objects of detailed study.  A quantity that often arises in
understanding properties of an operator is its `norm'. Let $V, W$ be
normed spaces, and let $A:V \mapsto W$ be a linear map from $V$ to
$W$. The operator norm of $A$ is defined to be
\[ \norm{A}{\text{op}} = \text{sup}_{v \in V, v \neq \vec{0}}
~\frac{\norm{A(v)}{}}{\norm{v}{}}. \]

Any continuous linear operator from $\rr^n \mapsto \rr^m$ can
naturally be associated with a matrix $A$ of dimension $m \times
n$. We will be interested in studying the $\ell_q$ to $\ell_p$ norm of
a matrix, defined as
\[ \norm{A}{\qtop} = \max_{x \in \rr^n, x \neq \vec{0}}
~\frac{\norm{Ax}{p}}{\norm{x}{q}}. \]

Throughout, $p, q \ge 1$, and $\norm{x}{p}$ refers to the standard
$\ell_p$ norm of the vector $x$, namely
\[ \norm{x}{p} = (|x_1|^p + \dots +|x_n|^p)^{1/p}.\]

Computing the $\qtop$-norm of a matrix is a natural optimization
problem, but is known to be efficiently solvable only under very
limited settings of parameters $p,q$.  Further, for different values
of the parameters, the problem has very different flavors. When
$p=q=2$, computing the norm reduces to the extensively studied problem
of computing the largest singular value of a
matrix~\cite{matrix}. When $p=1$ and $q=\infty$, it turns out to be
the well-studied Grothendieck problem~\cite{grothendieck, alonnaor},
which is defined as
\[ \max_{x_i, y_i \in \{-1, 1\}} \sum_{i,j} a_{ij} x_i y_j. \]

By duality of $\ell_p$ spaces, it follows (see
Appendix~\ref{sec:lpspace-duality}) that
\[ \norm{A}{\qtop} = \norm{A^T}{p' \mapsto q'}, \] where $A^T$ is the
transpose of the matrix $A$, and $p'$ and $q'$ are the `duals' of $p,
q$ respectively (i.e., we have, for instance $1/p + 1/p' = 1$). Thus
computing $\qtop$ norm is related to computing the $p' \mapsto q'$
norm in general.

We study the question of approximating $\norm{A}{\qtop}$ for different
ranges of the parameters $p, q$. The case $p=q$ is referred to as the
matrix $p$-norm (denoted by $\norm{A}{p}$), and has been considered in
the scientific computing community. For instance, it is known to have
connections with matrix condition number estimates (see \cite{higham}
for other applications). Another case which has been
studied~\cite{boyd, daureen} is one where the entries of the matrix
$A$ are restricted to be non-negative. Such instances come up in graph
theoretic problems, like in the $\ell_p$ oblivious routing question of
\cite{racke}.

\paragraph{Matrix $p$-norm.} For computing matrix $p$-norms,
polynomial time algorithms for arbitrary $A$ are known to exist only
for $p = 1, 2,$ and $\infty$. A simple way to approximate the $p$-norm
in general is by computing the vectors which maximize the $1, 2,$ and
$\infty$ norms of the matrix, and take the best of the three. It can
be shown, by applying extensions of H\"older's inequality (see
\cite{higham}) that this gives an $O(n^{1/4})$-approximation to the
$p$-norm. Recently, Steinberg~\cite{daureen} gives an algorithm with a
better approximation guarantee of $O(n^{25/128})$.\footnote{In fact,
  this approximation factor also applies to the problem of estimating
  $\norm{A}{\qtop}$ for $q \neq p$.}

However to the extent of our knowledge, the best inapproximability
results for any $p$ are due to recent independent work by
\cite{hendrix}, who show that it is NP-hard to compute the $p$-norm to
arbitrary relative precision when $p \not\in \{1, 2, \infty\}$ (i.e.,
there cannot be a $(1+\del)$ approximation algorithm with run time
poly$(n,m, 1/\del)$).

\paragraph{Other $\qtop$ norms.} In general for $p,q$, on the
algorithms side, the best known approximation ratio is
$O(n^{25/128})$, as mentioned earlier. However for $p \le 2$, $q >2$,
Nesterov\cite{nesterov} shows that the problem can be approximated to
a constant factor (which can be shown to be $<2.3$), using a
semidefinite programming relaxation. When the matrix has only
non-negative entries, this relaxation can be shown to be
exact~\cite{daureen}. On the hardness front, the problem is known to
be NP-hard in the range $q \ge p \ge 1$~\cite{daureen}.

\subsection{Our Results}
\paragraph{Non-negative matrices.} We first consider the case of
matrices $A$ with non-negative entries. Here we prove that if $1 \le p
\le q$, then $\norm{A}{\qtop}$ can be computed in polynomial
time. More precisely we give an algorithm which gives a $(1+\del)$
approximation in time polynomial in $n, m$, and $\log(1/\del)$.

Thus in particular, we give the first poly time guarantee (to the best
of our knowledge) for computing the matrix $p$-norm for non-negative
matrices. We give an analysis of a power iteration type algorithm for
computing $p$-norms proposed by Boyd~\cite{boyd}. More precisely, the
algorithm performs a fixed point computation, which turns out to mimic
power iteration for eigenvalue computations.

Heuristic approaches to many optimization problems involve finding
solutions via fixed point computations. Our analysis proves polynomial
convergence time for one such natural fixed point algorithm. These
techniques could potentially be useful in other similar settings.

We believe that this algorithm could be useful as an optimization tool
for other problems with objectives that involve $p$-norms (or as a
natural extension of eigenvalue computations). We now mention one such
application, to oblivious routing in the $\ell_p$ norm.

\paragraph{Application to Oblivious Routing.}
The Oblivious routing problem is a multicommodity flow problem where,
given a graph $G(V,E)$, we are asked to provide a routing algorithm by
specifying unit flows for every pair of vertices. For a set of
demands, the flow is routed by scaling the unit flows by the
corresponding demands. The quality of this flow is compared with the
best flow that routes these demands in hindsight according to some
objective (say congestion). When the objective is the $\ell_\infty$
norm (congestion), a beautiful result of \cite{racke1} gave an
algorithm to find a $O(\log n)$ competitive scheme. Englert and
R\"acke \cite{racke} recently showed that there exists an Oblivious
routing scheme which attains a competitive ratio of $O(\log n)$ when
the objective function is the $\ell_p$-norm of the flow vector ($|E|$
dimensional vector). Through a clever use of minmax duality in
zero-sum games, they reduced this problem of showing the existence of
such a scheme to $\ell_\infty$ case. However, they can efficiently
compute this oblivious routing scheme in polynomial time only for the
Euclidean norm ($p=2$).

As a by-product of our analysis, we can prove that in matrices with
strictly positive entries there is a unique maximum, to which our
algorithm converges. Using this and a related idea we develop
(Section~\ref{sec:stability}), we can make the result of \cite{racke}
constructive and efficiently find a $O(\log n)$-competitive Oblivious
routing scheme for all $\ell_p$-norms ($p \geq 1$).

\paragraph{Hardness  of approximation.}
In contrast, for general matrices (with negative entries allowed), we
show the inapproximability of \emph{almost polynomial factor} for
computing the $\qtop$ norm of general matrices when $q \geq p > 2$.

More precisely, we prove that it is NP-hard to approximate the the
$\qtop$ matrix norm to any constant factor. Under the stronger
assumption that $\mathsf{NP} \notin \mathsf{DTIME}(2^{polylog(n)})$,
we prove it is hard to approximate within a factor of $\Omega(2^{(\log
  n)^{1-\epsilon}})$ when $q \geq p > 2$.

For the $\ptop$ norm, we first show a constant factor hardness by a
gadget reduction from the gap version of MaxCut. Then we show that the
$\ptop$ norm multiplies under tensoring, and thus we get the desired
hardness amplification. While the proof of the small constant hardness
carries over to the $\qtop$ norm case with $q > p >2$, in general
these norms do not multiply under tensoring. We handle this by giving
a way of starting with a (tensored) hard instance of $\ptop$ norm
computation, and convert it to one of $\qtop$ norm computation.

When $q=\infty$, computing $\norm{A}{\infty \mapsto p}$ has a very simple alternate formulation (Definition~\ref{defn:lvp}): given vectors $\mathbf{a_1},\mathbf{a_2},\dots,\mathbf{a_n}$, we want to find the $\{\pm\}$ combination of the vectors (adding or subtracting the vector) which maximizes the $\ell_p$ norm. We show that the previous hardness result also extends to the case when $q=\infty$. 

We find the hardness results interesting because the bounds are very
similar to hardness for label cover, and it applies to a natural
numeric optimization problem.

\paragraph{Open directions.} While in the range where $p\leq q$, we have obtained a polynomial time algorithm to compute $\norm{A}{\qtop}$ when $A$ is non-negative, and obtained an almost polynomial factor hardness when $q\geq p$, we leave the question unanswered when $q<p$. Such hypercontractive norms have been studied in analysis and probability theory \cite{beckner,freidgut} and have also found prior use in proofs of lower bounds and hardness of combinatorial problems like the unique games. For instance, hypercontractive graphs (constant hypercontractive norm) are also integrality gap instances for unique games \cite{khot,ragh}. We believe that understanding the computability of hypercontractive norms of a matrix could also reveal interesting insights into the approximability of problems like the small set expansion, planted dense $k$-subgraph problem and the unique games conjecture. \anote{this is too sweeping - we need to word it carefully}. For instance, efficient algorithms for getting good approximations to $\norm{A}{\qtop}$ imply the current best algorithms for finding planted dense $k$-subgraphs in random graphs \cite{dks}. Hence, understanding the approximability of hypercontractive norms could throw light on the approximability of the dense-k subgraph. 

\paragraph{Comparision with previous work.}
For clarity, let us now tabulate our algorithmic and hardness results
in Tables~\ref{table:old,table:new} and show how they compare with known results for different values of
the parameters $p,q$.
\begin{table}[h]\label{table:old}
\caption{\textbf{Previous work:} on polynomial time approximation algorithms. NP-hardness just rules out exact polynomial time algorithms}
\begin{tabular}{|c|c||c|c|c|} 
\hline
	    & & $1<q<2$ & $q=2$ & $q>2$ \\
\hline
Algorithm    &$1<p<2$& poly(n)& constant factor \cite{nesterov}&  constant factor \cite{nesterov}\\
All $a_{ij} \geq 0$&&&Exact \cite{daureen}& Exact \cite{daureen} \\
Hardness	&&NP-hard when $p < q$ & NP-hard & NP-hard\\
\hline
Algorithm    &$p=2$ & poly(n)& Exact & constant factor \cite{nesterov} \\
All $a_{ij} \geq 0$&&&Exact&Exact \cite{daureen} \\
 Hardness&&&&NP-hard\\
\hline
Algorithm    &$p>2$ & poly(n)& poly(n)& poly(n)\\
All $a_{ij} \geq 0$&&&& \\
 Hardness&&&&NP-hard when $p<q$\\
\hline
\end{tabular}
\caption{\textbf{Our results.} $\beta(n)=2^{(\log n)^{1-\epsilon}}$ (almost polynomial).}
\begin{tabular}{|c|c||c|c|c|}
\hline
	    & & $1<q<2$ & $q=2$ & $q>2$ \\
\hline
Algorithm    &$1<p<2$& & & \\
All $a_{ij} \geq 0$&&\textbf{Exact if $p \leq q$}&Exact& Exact\\
Hardness	&& $\beta(n)-hard$&&\\
\hline
Algorithm    &$p=2$ & & & \\
All $a_{ij} \geq 0$&&&Exact&Exact\\
 Hardness&&&&\\
\hline
Algorithm    &$p>2$ &&&\\
All $a_{ij} \geq 0$&&&& \textbf{Exact if $p \leq q$} \\
 Hardness&&&&$\beta(n)$-hard if $p \leq q$\\
\hline
\end{tabular}
\end{table}
\paragraph{Related work.}
On a related front, the $\norm{A}{p \mapsto 2}$ is a special case of the $L_p$ Grothendieck problem which has been studied earlier by \cite{naor}. The problem is to 
\[\max_{||\mathbf{x}||_{p}\leq 1} \mathbf{x}^t B \mathbf{x} \]
\cite{naor} give an optimal (assuming UGC) $O(p)$ approximation algorithm (computing the $\norm{A}{p \mapsto 2$ is the $L_p$ Grothendieck problem for psd matrices). Further, there are also constant factor approximation algorithms in this range de to \cite{nesterov}. The $\infty \mapsto 1$ is the famous Grothendieck problem \cite{an} while the $\infty \mapsto 2$ norm reduces to maximizing a quadratic form for p.s.d matrices \cite{cw,nesterov}. \cite{madhur} studies an optimization problem with an $\ell_p$ norm objective - however they try to find the best subspace approximation of dimension $k$. When $k=n-1$ this can be shown to reduce to the $L_p$ Grothendieck problem for the matrix $A^{-1}$.
 
\subsection{Notation and Simplifications}\label{sec:intro:notation}

We write $\rplus$ for the set of non-negative reals. For a matrix $A$,
we let $A_i$ denote the $i$th row of $A$. Also $a_{ij}$ denotes the
element in the $i$th row and $j$th column. Similarly for a vector
$\xx$, we denote the $i$th co-ordinate by $x_i$. We say that a vector
$\xx$ is {\em positive} if the entries $x_i$ are all $>0$. Finally,
for two vectors $\xx,\yy$, we write $\xx \propto \yy$ to mean that
$\xx$ is {\em proportional to} $\yy$, i.e., $\xx = \lambda \yy$ for
some $\lambda$ (in all places we use it, $\lambda$ will be $>0$).

Matrices with non-negative entries to matrices with strictly positive
entries.\bnote{Move a paragraph from later...}

\subsection{Paper Outline} \label{sec:intro:outline}

\bnote{Update in case things are pushed to appendix!}  We start in
Section~\ref{sec:algo} by presenting the main algorithmic contribution
of the paper. In Section~\ref{sec:alg:description}, we describe the
algorithm, and then prove that it converges in polynomial number of
iterations to the optimum.

Then in Section~\ref{sec:alg:else}, we show some properties of the
optimization problem (like unique maximum, concavity around optimum)
which will be useful for an oblivious routing application, which we
present in~\ref{sec:oblivious}.

Finally in Section~\ref{sec:inapproximability}, we study the
approximability of the general problem, and prove the hardness results. 


